Federated Learning on Virtual Heterogeneous Data with Local-global Distillation

While Federated Learning (FL) is gaining popularity for training machine learning models in a decentralized fashion, numerous challenges persist, such as asynchronization, computational expenses, data heterogeneity, and gradient and membership privacy attacks. Lately, dataset distillation has emerged as a promising solution for addressing the aforementioned challenges by generating a compact synthetic dataset that preserves a model's training efficacy. However, we discover that using distilled local datasets can amplify the heterogeneity issue in FL. To address this, we propose Federated Learning on Virtual Heterogeneous Data with Local-Global Dataset Distillation (FedLGD), where we seamlessly integrate dataset distillation algorithms into FL pipeline and train FL using a smaller synthetic dataset (referred as virtual data). Specifically, to harmonize the domain shifts, we propose iterative distribution matching to inpaint global information to local virtual data and use federated gradient matching to distill global virtual data that serve as anchor points to rectify heterogeneous local training, without compromising data privacy. We experiment on both benchmark and real-world datasets that contain heterogeneous data from different sources, and further scale up to an FL scenario that contains a large number of clients with heterogeneous and class-imbalanced data. Our method outperforms state-of-the-art heterogeneous FL algorithms under various settings. Our code is available at https://github.com/ubc-tea/FedLGD.

==> img/cifar10Con_hist/cifar10Con.tex <==
\begin{figure}[ht]
	\centering
	\subfloat[]{  
		\includegraphics[width=0.3\linewidth]{img/cifar10Con_hist/0.png}}
	\subfloat[]{
	\includegraphics[width=0.3\linewidth]{img/cifar10Con_hist/1.png}}
	\subfloat[]{
		\includegraphics[width=0.3\linewidth]{img/cifar10Con_hist/2.png}}
  
	\subfloat[]{
		\includegraphics[width=0.3\linewidth]{img/cifar10Con_hist/3.png}}
        \subfloat[]{
		\includegraphics[width=0.3\linewidth]{img/cifar10Con_hist/4.png}}
        \subfloat[]{
		\includegraphics[width=0.3\linewidth]{img/cifar10Con_hist/5.png}}
	\caption{Visualization of the global and local distilled images from the first six clients of the Cifar10C dataset.}
\end{figure}

==> img/img_show/digitsCon_hist.tex <==
\begin{figure}[h]
	\centering
	\subfigure[MNIST]{  
		\includegraphics[width=0.45\linewidth]{img/digitCon_hist/0.png}}
	\subfigure[SVHN]{
	\includegraphics[width=0.45\linewidth]{img/digitCon_hist/1.png}}\\
 
	% \subfigure[USPS]{
	% 	\includegraphics[width=0.45\linewidth]{img/digitCon_hist/2.png}}
	% \subfigure[SynthDigits]{
	% 	\includegraphics[width=0.45\linewidth]{img/digitCon_hist/3.png}}

 %        \subfigure[MNIST-M]{
	% 	\includegraphics[width=0.45\linewidth]{img/digitCon_hist/4.png}}
	\caption{Histogram for the frequency of each RGB value in condensed \textit{DIGITS}. One can observe the distributions are very different. Note that figure (a) and figure (b) are both greyscale images with most pixels lies in 0 and 255.}
		\label{fig1}
\end{figure}


==> img/img_show/retinaCon_hist.tex <==
\begin{figure}[h]
	\centering
	\subfigure[]{  
		\includegraphics[width=0.45\linewidth]{img/retinsCon_hist/0.png}}
	\subfigure[]{
	\includegraphics[width=0.45\linewidth]{img/retinsCon_hist/1.png}}\\
 
	\subfigure[]{
		\includegraphics[width=0.45\linewidth]{img/retinsCon_hist/2.png}}
	\subfigure[]{
		\includegraphics[width=0.45\linewidth]{img/retinsCon_hist/3.png}}
	\caption{Histogram for the frequency of each RGB value in \textit{Retina}. The red bar represents the count for R; the green bar represents the frequency of each pixel for G; the blue bar represents the frequency of each pixel for B. (a) Drishti; (b) Kaggle; (c) RIM; (d)REFUGE.}
		\label{fig1}
\end{figure}
